Lindstrom theorems for fragments of first-order logic

Lindstr\"om theorems characterize logics in terms of model-theoretic conditions such as Compactness and the L\"owenheim-Skolem property. Most existing characterizations of this kind concern extensions of first-order logic. But on the other hand, many logics relevant to computer science are fragments or extensions of fragments of first-order logic, e.g., k-variable logics and various modal logics. Finding Lindstr\"om theorems for these languages can be challenging, as most known techniques rely on coding arguments that seem to require the full expressive power of first-order logic. In this paper, we provide Lindstr\"om theorems for several fragments of first-order logic, including the k-variable fragments for k>2, Tarski's relation algebra, graded modal logic, and the binary guarded fragment. We use two different proof techniques. One is a modification of the original Lindstr\"om proof. The other involves the modal concepts of bisimulation, tree unraveling, and finite depth. Our results also imply semantic preservation theorems.

==> letter.tex <==
Dear Balder ten Cate,

Please find enclosed a version of your paper "Lindström theorems for
fragments of first-order logic" formatted for the Journal.

We prefer not to use ``\sloppy'' as a global option, but rather deal
with spacing issues at the level of individual paragraphs.

Only two such problems arose: which can be solved with slight
reformulations:

page 22, paragraph before Fact 3.5.
page 24, first two paragraphs.

In addition, I've attempted to improve the displays in the proof of
the claim on page 5 and in the proof of Lemma 3.18 on page 17.

I hope that these modifications are acceptable.  In case you have
other corrections or changes, just let me know directly.

One remark concerning the included graphics: in the future you may
want to consider the PGF/TikZ package by Till Tantau (author of the
beamer package), see, e.g., http://www.texample.net/tikz/examples/

Sincererly yours,

-- Jürgen Koslowski
   LMCS Layout Editor

